SARS-CoV-2 orthologs of pathogenesis-involved small viral RNAs of SARS-CoV

Background: The COVID-19 pandemic clock is ticking and the survival of many of mankind's modern institutions and or survival of many individuals is at stake. There is a need for treatments to significantly reduce the morbidity and mortality of COVID-19. Hence, we delved deep into the SARS-CoV-2 genome, which is the virus that has caused COVID-19. SARS-CoV-2 is from the same family as SARS-CoV in which three small viral RNAs (svRNA) were recently identified; those svRNAs play a significant role in the virus pathogenesis in mice. Contribution: In this paper, we report potential orthologs of those three svRNAs in the SARS-CoV-2 genome. Instead of off-the-shelf search and alignment algorithms, which failed to discover the orthologs, we used a special alignment scoring that does not penalize C/T and A/G mismatches as much as the other mutations. RNA bases C and U both can bind to G; similarly, A and G both can bind to U, hence, our scoring. We also validate this hypothesis using a novel, independent computational experiment. To validate our results, we confirmed the discovered orthologs are fully conserved in all the tested publicly available genomes of various strains of SARS-CoV-2; the loci at which the SARS-CoV-2 orthologs occur are close to the loci at which SARS-CoV svRNAs occur. We also report potential targets for these svRNAs. We hypothesize that the discovered orthologs play a role in pathogenesis of SARS-CoV-2, and therefore, antagomir-mediated inhibition of these SARS-CoV-2 svRNAs inhibits COVID-19.

==> Drawings.tex <==
\figureDefinition{svRNA1}
\figureExtension{png}
\figureDescription{Alignment of the first svRNA in SARS-CoV and its identified ortholog in SARS-CoV-2.}
\figureOptions{scale=0.5}
\figureCaption{Alignment of the first svRNA in SARS-CoV and its identified ortholog in SARS-CoV-2. Top: nsp3.1 svRNA sequence GAGGAAGAAGAGGACGAT in SARS-CoV according to \cite{morales2017sars}. Bottom: Ortholog of nsp3.1 svRNA sequence GATGAAGAAGAAGGTGAT in SARS-CoV-2. $|$ represents a match, $-$ represents a gap (indel), empty represents a mismatch, and $:$ represents a non-detrimental mismatch.}

\figureDefinition{svRNA2}
\figureExtension{png}
\figureDescription{Alignment of the second svRNA in SARS-CoV and its identified ortholog in SARS-CoV-2.}
\figureOptions{scale=0.5}
\figureCaption{Alignment of the second svRNA in SARS-CoV and its identified ortholog in SARS-CoV-2. Top: nsp3.2 svRNA sequence GAGGAAGAAGAAGAGGAAGACT in SARS-CoV according to \cite{morales2017sars}. Bottom: Ortholog of nsp3.2 svRNA sequence GAAGAAGAGCAAGAAGAAGATT in SARS-CoV-2. $|$ represents a match, $-$ represents a gap (indel), empty represents a mismatch, and $:$ represents a non-detrimental mismatch.}


\figureDefinition{svRNA3}
\figureExtension{png}
\figureDescription{Alignment of the third svRNA in SARS-CoV and its identified ortholog in SARS-CoV-2.}
\figureOptions{scale=0.5}
\figureCaption{Alignment of the third svRNA in SARS-CoV and its identified ortholog in SARS-CoV-2. Top: N svRNA sequence AGGAACTGGCCCAGAAGCTTC in SARS-CoV according to \cite{morales2017sars}. Bottom: Ortholog of N svRNA sequence AGGAACTGGGCCAGAAGCTGGAC in SARS-CoV-2. $|$ represents a match, $-$ represents a gap (indel), empty represents a mismatch, and $?$ represents a potential omission. It is possible that some or all of the last four (4) nucleotides GGAC of the bottom sequence are dropped (omitted).}

%\annotationDefinition{svRNA1}
%\annotationName{svRNA1}
%\annotationDescription{a widget in the Visio drawing}
%\annotationDefinition{Thing}
%\annotationName{thing}
%\annotationDescription{a thing in the visio drawing}
%\annotationDefinition{WidgetThingConnection}
%\annotationName{connection}
%\annotationDescription{the arrow connecting the widget and the thing}


%\figureDefinition{VisioDrawing}
%\figureExtension{pdf}
%\figureDescription{is an example drawing created in Visio}

%\annotationDefinition{Widget}
%\annotationName{widget}
%\annotationDescription{a widget in the Visio drawing}
%\annotationDefinition{Thing}
%\annotationName{thing}
%\annotationDescription{a thing in the visio drawing}
%\annotationDefinition{WidgetThingConnection}
%\annotationName{connection}
%\annotationDescription{the arrow connecting the widget and the thing}

%\figureDefinition{TpXDrawing}
%\figureExtension{tpx}
%\figureCaption{PRIOR ART}
%\figureDescription{is an example drawing created in TpX}

%\annotationDefinition{input}
%\annotationName{input}
%\annotationDescription{the input}
%\annotationDefinition{output}
%\annotationName{output}
%\annotationDescription{the output}
%\annotationDefinition{mathProcessor}
%\annotationName{math processor}
%\annotationDescription{the math procesor}

